MeerKAT caught a Mini Mouse: serendipitous detection of a young radio pulsar escaping its birth sit

In MeerKAT observations pointed at a Galactic X-ray binary located on the Galactic plane we serendipitously discovered a radio nebula with cometary-like morphology. The feature, which we named `the Mini Mouse' based on its similarity with the previously discovered `Mouse' nebula, points back towards the previously unidentified candidate supernova remnant G45.24$+$0.18. We observed the location of the Mini Mouse with MeerKAT in two different observations, and we localised with arcsecond precision the 138 ms radio pulsar PSR J1914+1054g, recently discovered by the FAST telescope, to a position consistent with the head of the nebula. We confirm a dispersion measure of about 418 pc cm$^{-3}$ corresponding to a distance between 7.8 and 8.8 kpc based on models of the electron distribution. Using our accurate localisation and 2 period measurements spaced 90 days apart we calculate a period derivative of (2.7 $\pm$ 0.3) $\times$ 10 $^{-14}$ s s$^{-1}$. We derive a characteristic age of approximately 82 kyr and a spin down luminosity of 4$\times$10$^{35}$ erg s$^{-1}$, respectively. For a pulsar age comparable with the characteristic age, we find that the projected velocity of the neutron star is between 320 and 360 km/s if it was born at the location of the supernova remnant. The size of the proposed remnant appears small if compared with the pulsar characteristic age, however the relatively high density of the environment near the Galactic plane could explain a suppressed expansion rate and thus a smaller remnant.

==> def_bibtex.tex <==
\def\apj{ApJ}
\def\apjs{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\araa{Annual Reviews}
\def\apss{Ap\&SS}
\def\atel{The Astronomer's Telegram}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\ssr{Space Science Reviews}
\def\prd{Physical Review D}
\def\pasp{Publications of the Astronomical Society of the Pacific}
\def\na{New Astronomy}



